Using Audio Data to Facilitate Depression Risk Assessment in Primary Health Care

Telehealth is a valuable tool for primary health care (PHC), where depression is a common condition. PHC is the first point of contact for most people with depression, but about 25% of diagnoses made by PHC physicians are inaccurate. Many other barriers also hinder depression detection and treatment in PHC. Artificial intelligence (AI) may help reduce depression misdiagnosis in PHC and improve overall diagnosis and treatment outcomes. Telehealth consultations often have video issues, such as poor connectivity or dropped calls. Audio-only telehealth is often more practical for lower-income patients who may lack stable internet connections. Thus, our study focused on using audio data to predict depression risk. The objectives were to: 1) Collect audio data from 24 people (12 with depression and 12 without mental health or major health condition diagnoses); 2) Build a machine learning model to predict depression risk. TPOT, an autoML tool, was used to select the best machine learning algorithm, which was the K-nearest neighbors classifier. The selected model had high performance in classifying depression risk (Precision: 0.98, Recall: 0.93, F1-Score: 0.96). These findings may lead to a range of tools to help screen for and treat depression. By developing tools to detect depression risk, patients can be routed to AI-driven chatbots for initial screenings. Partnerships with a range of stakeholders are crucial to implementing these solutions. Moreover, ethical considerations, especially around data privacy and potential biases in AI models, need to be at the forefront of any AI-driven intervention in mental health care.

==> scratch.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Feature} & \textbf{Metric} & \textbf{Depression diagnosis} & \textbf{No depression diagnosis} \\
\hline
\multirow{MFCC Mean} & Mean & -74.43 & -75.08 \\
& SD & 7.67 & 7.25 \\
\hline
\multirow{Spectral Centroid} & Mean & 0.0785 & 0.0792 \\
& SD & 0.0261 & 0.0225 \\
& Count & 1632 & 2337 \\
\hline
\multirow{Spectral Complexity} & Mean & 37.66 & 29.80 \\
& SD & 31.89 & 31.09 \\
\hline
\multirow{Zero Crossing Rate} & Mean & 0.0541 & 0.0551 \\
& SD & 0.0173 & 0.0199 \\
\hline
\end{tabular}
\caption{Descriptive statistics for features by group.}
\label{tab:feature_stats}
\end{table*}



